A Survey on Time-Series Distance Measures

Distance measures have been recognized as one of the fundamental building blocks in time-series analysis tasks, e.g., querying, indexing, classification, clustering, anomaly detection, and similarity search. The vast proliferation of time-series data across a wide range of fields has increased the relevance of evaluating the effectiveness and efficiency of these distance measures. To provide a comprehensive view of this field, this work considers over 100 state-of-the-art distance measures, classified into 7 categories: lock-step measures, sliding measures, elastic measures, kernel measures, feature-based measures, model-based measures, and embedding measures. Beyond providing comprehensive mathematical frameworks, this work also delves into the distinctions and applications across these categories for both univariate and multivariate cases. By providing comprehensive collections and insights, this study paves the way for the future development of innovative time-series distance measures.

==> section/S12_Evaluation.tex <==
\section{Evaluation}
In this section, we will first introduce the existing representative work that evaluating the efficiency of distance measure under univariate or multivariate cases. To measure the effectiveness of distancem measures, one of the widely adapted method is utilizing one-neartest neighbor classifier which applies distance measure to compare each test data with all training data and assign the label of closes training data as the predicted label of test data. After obtaining the predicted label for all test data, different evaluation metrics such as classification accuracy can be applied to measure the effectiveness. Once the accuracy is obtained, the pair-wise comparison performed by Wilcoxon test and Criticial Difference (CD) Diagram generated using average rank provided by Friedman-Nemenyi test are commonly applied to ensure the rigorousness of statistical anlysis. \todo{Continue: Add more information and chatGPT rewrite.}
\subsection{Univariate Distance Measures Evaluation}

\subsection{Multivariate Distance Measures Evaluation}
